Correspondence Networks with Adaptive Neighbourhood Consensus

In this paper, we tackle the task of establishing dense visual correspondences between images containing objects of the same category. This is a challenging task due to large intra-class variations and a lack of dense pixel level annotations. We propose a convolutional neural network architecture, called adaptive neighbourhood consensus network (ANC-Net), that can be trained end-to-end with sparse key-point annotations, to handle this challenge. At the core of ANC-Net is our proposed non-isotropic 4D convolution kernel, which forms the building block for the adaptive neighbourhood consensus module for robust matching. We also introduce a simple and efficient multi-scale self-similarity module in ANC-Net to make the learned feature robust to intra-class variations. Furthermore, we propose a novel orthogonal loss that can enforce the one-to-one matching constraint. We thoroughly evaluate the effectiveness of our method on various benchmarks, where it substantially outperforms state-of-the-art methods.

==> append_gm.tex <==
\onecolumn
\appendix
\section*{Appendices}


\subsection{Introduction}

Estimating dense correspondence is a fundamental problem which has seen variety of applications in object detection~\cite{Duchenne_ICCV11,Liu_PAMI11_SIFTFlow}, human pose, action recognition~\cite{Yao_ECCV12_ActionRecognition,Guo_ECCV18_NeuralGM}  
and data association for camera motion estimation or 3D model reconstruction~\cite{Yang_PR17_Correspondence3OGM,Torresani_ECCV08_CorrespondenceGM,Agarwal_ICCV09_BuildRome,Sattler_CVPR17_Benchmark_6DOF}. Recent state-of-the-art methods have dealt with the problem using deep Convolutional Neural Network (CNN), for example, training CCN feature backbone to produce identical features at correspondent key points~\cite{Choy_NIPS16_UCN} or maximising the correlation between the feature maps with enforced regional consistency known as the Neighbourhood Consensus (NC-Net)~\cite{Rocco_NIPS18_NCNet,Huang_ICCV19_DCCNet}. Thank to highly descriptive CNN, these data-driven approaches are by far more accurate than conventional method including the SiftFlow~\cite{Liu_PAMI11_SIFTFlow} methods  neural networks which can be solved with labelled training data. However, these methods often reinvent the wheel and results in models containing many redundant parameters. For example, the neighbourhood consensus filtering in~\cite{Rocco_NIPS18_NCNet} is equivalent to perform the convolution over the $\epsilon$-graph generated over the associated nodes between two graphs. The spacial context encoding~\cite{Huang_ICCV19_DCCNet} is another example highly relevant to the pairwise term in graph matching, yet the spatial encoding repeatedly manipulates the correlation map results in significant redundancy.

In this paper, we first review the popular correspondence network from the classic graph matching perspective and bridge the gap between the two research areas running parallel for a long time. As a result, we take inspiration from both ends and makes the following contributions:
\begin{itemize}
\item first, inspired by GM, we replace the spatial context encoding with a convolutional edge feature extractor, which has wider receptive field and contains less redundancy but more effective than the former. 
\item second, to avoid dealing with extra large adjacency matrix in GM, we project the edge features on node adjacency matrix and strengthen the neighbourhood consensus filtering with the capability of adapting to different scales of receptive fields in source or target images. 
\item third, inspired by tho orthogonal constraint in graph matching~\cite{Jiang_AAAI17_NOGM}, we introduce a novel orthogonal loss which softly penalises the many-to-one correspondences and can be flexibly deployed with either a weak or strong supervision.   
\end{itemize}
When combined together, above modules result in a novel deep correspondence network architecture that outperforms the state-of-the-art which will be demonstrated in the experimental section. Figure~\ref{fig:overview} illustrates how the proposed method works during inference with main contributions highlighted in the yellow text-boxes.

\begin{figure*}[t]
% this figure should cross two columns and appear on the top of the second page
\begin{center}
   \includesvg[width=0.8\textwidth]{image/main}
\end{center}
   \caption{Overview of the approach. The red and blue modules are related to features extracted from the source and target images, respectively. These features are nodewise features directly extracted from a fixed standard backbone feature extractor and edgewise features describing the edges in each image. Both sets of features are then correlated to form the adjacency matrices which are then refined by the adaptive neighour consensus module. The refined adjacency is the final output of the system. Given a query key point, the 4 nearest neighbours can be retrieved from it and combined into a low resolution correlation map, from which the predicted key points can be retrieved from it.}
\label{fig:overview}
\end{figure*}

\section{Problem Formulation}\label{sec:gm}
Graph Matching (GM) aims to find correspondences between the nodes of two different graphs, subject
to a one-to-one mapping constraint, such that each node has at most one correspondence.
It is typically solved as a Binary Quadratic Problem 
(BQP)~\cite{Leordeanu_ICCV05_SM,Cour_NIPS06_SMAC,Minsu_ECCV10_RRWM,Zhou_CVPR12_FGM,Jiang_AAAI17_NOGM,FudongECCV18_AdaptiveTransform}. GM is highly related to the dense correspondence problem. In this section, we first briefly review the BQP and interpret existing deep neural network in terms of GM. Then, we derive a novel edgewise term which inspires the convolutional edgewise feature extractor.

A graph can be denoted as a set $\mathcal{G} = (\mathcal{V},\mathcal{E}, \mat{U}, \mat{F})$, where $\mathcal{V}$ 
is a set of nodes, $\mathcal{E}\subset{\mathcal{V}\times\mathcal{V}}$ 
a set of of edges connecting two nodes. For example,  $e = (i,j)$ connecting nodes $i$ and $j$.
$\mat{U}\in\mathbb{R}^{|\mathcal{V}|\times d}$ is a matrix of nodewise features, where $|\mathcal{V}|$ is the cardinality of
$\mathcal{V}$ and $d$ is the feature dimensionality. $\mat{F}\in\mathbb{R}^{|\mathcal{E}|\times d}$ is the matrix of edgewise features matrix\footnote{Without losing of generality, we use $d$ to denote the dimensionality of both edgewise and nodewise features. In experiments, they are different.}.

The GM is to find the node correspondence between two graphs $\mathcal G$ and $\mathcal G^\prime$ which can be represented by a binary assignment matrix $\mat{X}\in\{0,1\}^{|\mathcal{V}|\times|\mathcal{V}'|}$, where $\mathbf{X}_{i,i'}=1$ if the 
$i$-th node in $\mathcal{G}$ and $i'$-th node in $\mathcal{G}^\prime$ are a pair of correspondent nodes, 
otherwise $\mathbf{X}_{i,i'}=0$. It can be solved by maximising the following quadratic objective function:
\begin{equation}
f(\mat X) = vec(\mat{X})^\top \mat{K}vec(\mat{X}) \text{ }s.t.\text{ } \mat X \vect 1 \leq \vect{1} \text{, } \mat X^\top \vect{1}\leq \vect{1} \label{eq:bqp}
\end{equation}

where $\text{vec}(\mat{X})$ vectorise $\mat{X}$ in the column-major order, and
$\mat{K} \in \mathbb{R}^{|\mathcal{V}||\mathcal{V}'|\times|\mathcal{V}||\mathcal{V}'|}$ is the
similarity matrix\footnote{$\mat K$ is also known as the affinity matrix or adjacency matrix over the association graph.}.
Specifically, the elements on the main diagonal $\mat{K}_{ij,i'j'}$ measure the node similarity
between the $i\in\mathcal{V}$ and $i'\in\mathcal{V}^\prime$ and the off-diagonal elements
$\mat{K}_{ij,i'j'}$ measure the edgewise similarity between $(i,j)\in\mathcal{E}$ and
$(i',j')\in\mathcal{E}^\prime$. Solving Equation~\ref{eq:bqp} is NP-hard but can be approximately solved using the power iteration algorithm~\cite{Leordeanu_ICCV05_SM}. However, $\mat{K}$ can be huge in size but sparse. As a result, $\mat{K}$ is often factorised into two smaller but denser node and edge adjacency matrix~\cite{Zhou_CVPR12_FGM,Zanfir_CVPR18_DeepGM}:
\begin{equation}
    \mat{K} =[\fvec(\mat{K}_n)]+(\mat{G}'\otimes \mat{G} )[\fvec(\mat{K}_e)](\mat{H}'\otimes \mat{H} )^\top \label{eq:fac}
\end{equation}
where $\mat{K}_n\in\mathbb{R}^{|\mathcal{V}|\times|\mathcal{V}'|}$ is the node adjacency matrix whose elements $\mat K_{n,i,i'}$ describes the similarity between the node $i\in\mathcal V$ and node $i'\in\mathcal V'$. Similarly, and $\mat{K}_e\in\mathbb{R}^{|\mathcal{E}|\times|\mathcal{E}'|}$ describes the edge similarity. $\mat{G}\in\{0,1\}^{|\mathcal{V}|\times|\mathcal{E}|}$ are the incident matrices such that $\mat{G}_{i,j}=1$ if the
$j$-th edge leaves the $i$-th node and $\mat{H}\in\{0,1\}^{|\mathcal{V}|\times|\mathcal{E}|}$ such that $\mat{H}_{i,j}=1$ if the $j$-th edge enters the $i$-th node. $\otimes$ is the Kronecker product and $[\vect{x}]$ represents a diagonal matrix with $\vect{x}$ on the main diagonal. 

It is worth noting that the first term in Equation~\ref{eq:fac} describes the contribution by node feature to the matching and the second term describes the contribution of edge features to the matching.   


\subsection{Related work}

%\subsection{Connection with deep correspondence networks}
There are large volume of works~\cite{Choy_NIPS16_UCN,Zanfir_CVPR18_DeepGM,Rocco_NIPS18_NCNet,Huang_ICCV19_DCCNet} about establishing dense correspondences using deep CNN. UCN~\cite{Choy_NIPS16_UCN} one of the pioneering works match two views of a scene by training a standard feature backbone to produce descriptive deep features which can be compared directly to measure their similarity.  This approach can be formulated as $\mat K_n = c(vec(\psi(\mat I)), vec(\psi(\mat I')))$  where $\mat I$ and $\mat I'$ are the input images, $\psi()$ can be any feature extractor. $vec(.)$ vectorises the 2D feature map into 1D. $c(\vect{f},\vect{f}')$ represents a correlation measurement which can be either feature-wise cosine distance $\frac{\vect{f}^\top \vect{f}'}{\|\vect{f}\|^2_2\|\vect f'\|^2_2}$ or similarity function $\exp(\frac{\|\vect{f}-\vect{f}'\|^2_2}{\sigma^2})$. It can be seen that UCN sololy relies on node features, each node is matched independently to others and no edge features are considered.

GMN~\cite{Zanfir_CVPR18_DeepGM} integrates into UCN the differentiable GM layers converted from the power iteration algorithm and doubly-stochastic normalisation~\cite{Cour_NIPS06_SMAC}. It incooperates both node and pair features for matching. However, GMN remains heavily relies on the feature backbone for matching. Also, GMN directly manipulates the $\mat K$ which restrict its scalability. The doubly-stochastic layer requires the point pairs contains only one-to-one matches which is less competitive for establishing dense correspondences.

NC-Net~\cite{Rocco_NIPS18_NCNet, Huang_ICCV19_DCCNet} represents another group of CNN-based correspondence network which is capable of formulating dense correspondence using fixed pre-trained feature backbone. Specifically, it reshape the $\mat K_n$ into a 4D correlation map so that it can be filtered with a 4D convolutions. The 4D convolution essentially refines the correlation score by jointly consider the correlation within the neighbourhoods defined in both images. In addition, NC-Net also introduce a soft mutual matching layer which enforce the global constraints on top of the neighbourhood concensus. From GM perspective, the mutual matching layer can viewed as a soft doubly-stochastic normalisation and serves similar purpose. %(better to shown with equations)

NC-Net and its variants has seen great improvements and are more scalable than directly converting GM into differentiable layers~\cite{Zanfir_CVPR18_DeepGM, } to the dense correspondence problem and incorporate the ideas analogous to GM, however, it mainly operates on the domain of $\mat K_n$. In this paper, we introduce a novel edge feature extractor to incooperate the edge adjacency $\mat K_e$ to determine the matching. 

To keep the low-dimensionality of $\mat K_n$, we show that $\mat K_e$ can be projected into the domain of $\mat K_n$ which inspires the idea of CNN-based edge extractor avoiding dealing with the large sparse matrix $\mat G$ and $\mat H$ which will be described in the next section. 


\subsection{Method}

$\mat K_n$ and $\mat K_e$ encodes nodewise and edgewise similarity, respectively. As the node adjacency is usually smaller than the edge adjacency and the edges takes extra effort to construct, it is ideal if it exits a projection $\mathcal T:\mathbb{R}^{|\mathcal{E}|\times|\mathcal{E}'|} \rightarrow \mathbb{R}^{|\mathcal{V}|\times|\mathcal{V}'|}$ i.e. can project $\mat K_e$ into $\mat K_n$.   

\subsection{Deriving $\mathcal T$}

Similar to $\mat{K}_n$ which is a function of the node features, $\mat{K}^e$ can be derived as a function of edge features $\mat F$ and $\mat F'$ using the following equation~\cite{Zhou_CVPR12_FGM}:
\begin{equation}
\mat{K}^\prime_q(\mat{F}_1, \mat{F}_2) = \sum_i \mat{A}_i^1 \mat{S} \mat{A}_i^2  \label{eq:kprime}
\end{equation}
where $\mat{S}\in\mathbb{R}^{|\mathcal{V}_1|\times|\mathcal{V}_2|}$ is a uniform bi-stochastic 
assignment matrix, $\mat{A}_i = \mat{G}[\vect{f}_{i}]\mat{H}^\top$, and $\vect{f}_{i}$ is the 
$i^{\text{th}}$ column of $\mat{F}$. 

\subsection{Network}

If we regard the edge attributes as the output of a function $\phi:\mathbb{R}^d\times\mathbb{R}^d\rightarrow\mathbb{R}^d$ that takes two
node attribute vectors, i.e. $\vect{f}=\phi(\vect u_i, \vect u_j)$, where $\vect u_i$ and $\vect u_j$ are the two columns in the node attribute matrix $\mat U$
, we can then express $\mat{K}_q^\prime$ as a pure function of node attributes. In addition, it is apparent that $\mat{K}_p$ is also a function of $\mat{U}_1$ and $\mat{U}_2$, so we can derive that
\begin{align}
    \mat X &= \varphi^\prime(\mat K_p, \mat K_q ) = \varphi^\prime(\mat K_p(\mat U_1, \mat U_2), \mat K_q'(\mat F_1,\mat F_2) ) \notag\\
    &= \varphi^\prime(\mat K_p(\mat U_1,\mat U_2), \mat K_q^\prime(\phi(\mat U_1),\phi(\mat U_2)) = \psi(\mat U_1, \mat U_2) \label{eq:inter}
\end{align}
where $\psi$ is the overall hyper-function representing the whole network structure. In contrast,
previous approaches to deep GM reconstituted each step of classical GM methods into
differentiable layers.
We avoid being bounded by the structure and mathematical formulation of any particular
classical algorithm, and instead design a network that aims to implicitly capture 
the entire GM process as a whole.

Our network learns a feature extractor $\mat{U} = \zeta(\mat{I}, \mathcal V)$ where $\mat I$ is an image and $\mathcal V$ is the set of key-points for that image.
In our experiments, the network hyper-function $\psi$ takes the form of the function
\begin{equation}
    \psi(\mat{U}_1, \mat{U}_2) = \psi( \mat{U}_1\mat{\Lambda} \mat{U}_2^\top )
\end{equation}
where $\mat{\Lambda}$ is a diagonal matrix of learn-able weights.
% We found this to be an effective approximation of the ideal $\varphi'$, as it simple and quick to compute and 
% leads to state of the art results, as shown in our experimental section.

Our network architecture is shown in Figure \ref{fig:overview}. It follows the structure
of a Siamese convolutional regressor \cite{Doumanoglou_CORR16_Siamese} to predict the
assignment matrix $\mat{X}$. We use ResNet-50 as the encoder and a feature pyramid network as the decoder.
The decoder mainly serves as an up-sampler to provide higher resolution feature maps. 

\subsection{Orthogonal Loss}

The one-to-one mapping turns out to be a useful clue to improve the matching accuracy in classic graph matching. There are several methods to enforce the one-to-one constraint. For example, the predicted assignment matrix can be normalised into a bi-stochastic matrix \cite{Zanfir_CVPR18_DeepGM}, or one could optimise the graph matching objective function in Eq.~\ref{eq:bqp} with an affinity constraint that encodes the one-to-one constraint. Recent work~\cite{Jiang_AAAI17_NOGM} shows that optimising with the orthogonal constraint $\|\mat{X}\mat{X}^\top - \mat{I}\|_F=0$ guarantees the KKT optimality of the solution. 

All of the above methods works well for $|\mathcal V_1|=|\mathcal V_2|$, however, when one-to-none matches exist, the $\mat{X}\mat{X}^\top$ becomes a diagonal matrix with binary values. 
Instead, we introduce the novel orthogonal loss as follows
\begin{equation}
    \mathcal{L_\text{orth}} =  \|\mat{X} - \mat{X}_{gt}\|_F + \alpha\|\mat{X}\mat{X}^\top - \mat{X}_{gt}\mat{X}_{gt}^\top\|_F
\end{equation}
where $\alpha$ is balancing hyperparameter.
In all of our experiments, $\alpha$ is set to 0.1.
Critically, $\mat{X}_{gt}\mat{X}_{gt}^\top$ has zeros in its diagonal that allows both one-to-one and one-to-none matches to be accurately penalised.
As well, this formulation better separates positive assignments from negative assignments.
Placing the constraint in the loss, rather than implementing it as a layer in the network as in previous works \cite{Zanfir_CVPR18_DeepGM},
reduces the complexity of the network while improving its performance, as shown in our experiments.


\subsection{Experimental results}

% The broader statistics of our datasets are outlined in Table~\ref{tab:datastats}.
We perform our experiments on an Intel Core i7-6850K CPU with a Titan Xp GPU.
For the encoder-decoder, we use ResNet-50 with a feature pyramid network (FPN)~\cite{Lin_CVPR17_PFN}. The dimensionality for both the node features and edge features is 258, where the first 256 are from the feature extractor and the last 2 are the normalised pixel location. Specifically, the last 2 features are given by $(\mathbf p_i - \bar{\mathbf p})/s$, where $\mathbf p_i$ is the pixel location of the $i^{th}$ key-point, $\bar{\mathbf p}=\frac{1}{|\mathcal V|}\sum_{i\in\mathcal V}\mathbf p_i$ is the centroid of all the key-points, and $s=\frac{1}{|\mathcal V|}\sum_{i\in\mathcal V}\|\mathbf p_i-\bar{\mathbf p}\|_2$ is the mean distance from a key-point to its centroid. To compensate for the pixel displacement loss (d-loss) adopted in DeepGM, we also add a similar term into our loss: $\beta\|(\mat{X}_{gt}-\mat{X})\mat P_{gt}\|_2$, where $\mat P_{gt}\in\mathbb{R}^{n\times2}$ are the ground truth key-point locations and $\beta$ is another balance hyper-parameter ranging from 0.25 to 0.5. 

\subsection{Baselines}
Our baselines are: DeepGM; a variant of DeepGM combining ResNet-50 with FPN as well as the affinity matrix layer, power iteration layer, and the bi-stochastic layer; NC-Net~\cite{Rocco_NIPS18_NCNet}, a weakly supervised key-point matching method; WarpNet~\cite{Kanazawa_CVPR16_WarpNet} and UCN~\cite{Choy_NIPS16_UCN}, both model-based matching approaches; and several classic matching methods including SIFT flow~\cite{Liu_PAMI11_SIFT} and DSF~\cite{Kin_CVPR13_DSF}.

% \begin{table}[h]
%   \centering
%   \resizebox{\linewidth}{!}{
%   \begin{tabular}{lrrrrrr}\toprule
%   &\multicolumn{3}{c}{CUB}&\multicolumn{3}{c}{PASCAL VOC}\\
%   \cmidrule(r){2-4}\cmidrule(l){5-7}
%   &\multicolumn{1}{l}{Train}&\multicolumn{1}{l}{Val}&\multicolumn{1}{l}{Test}&
%   \multicolumn{1}{l}{Train}&\multicolumn{1}{l}{Val}&\multicolumn{1}{l}{Test}\\
%   \midrule
%   No. of Images         & 5,395 & 599    & 5,794     & 7,498     & 833       & 8,351 \\
%   Total No. of Pairs    & 14,44921 & 179,700    & 2,485,335 & 8,602,849 & 921,085   & 9,210,875 \\
%   No. of Valid Pairs    & 14,44921 & 179,700    & 5,000       & 5,824,516 & 633,213   & 633,2130 \\
%   \bottomrule
%   \end{tabular}}
%   \vspace{0.5em}
%   \caption{Dataset statistics for the CUB and PASCAL VOC datasets}
%   \label{tab:datastats}
% \end{table}

\subsection{Datasets}
\label{sec:expclass}
We conduct our experiments on Caltech-UCSD Birds-200-2011~\cite{Welinder_2010_CUB} (CUB), PASCAL VOC 2011~\cite{PASCAL_VOC} with Berkeley annotations~\cite{Lubomir_PAMI_Poselets}, and the Sintel dataset~\cite{Butler_ECCV12_Sintel}.

\subsubsection{CUB} This dataset contains 200 bird categories, consisting of 11,788 images, with bounding boxes and
up to 15 key-points.
In training we sample images randomly from the CUB-200-2011 training set.
Our validation set was generated by randomly taking 10\% from the training set, leaving the remaining 90\% 
for training. To make a fair comparison with our baselines, we limited our selection of pairs to those within 3 nearest neighbours on the pose graph of~\cite{krause2015fine}. 
Images are resized to $256\times256$ before being fed into the network.

\subsubsection{Pascal VOC with Berkeley annotations}
This key-point dataset is an extension of the PASCAL VOC 2011 dataset~\cite{Lubomir_PAMI_Poselets}.
The original dataset contains 20 image classes with a total of 30,629 annotated objects. Each object has a theoretical maximum
of 23 key-points, however the actual maximum number of key-points varies between the classes
(min: 6 -- potted plant, max: 23 -- person). In our experiments, we use the 
validation set  of the Berkely annotation images for testing and split the training data 9:1 to generate a training and 
validation set. Because of the vast number of pairs produced by combining images, to test on the dataset we randomly sample 5,000 pairs per epoch for testing all of our algorithms. 

The pairs of images are formed respecting class boundaries, discarding any image pairs where there are
less than 5 key-point matches.
This generates over 5M pairs of images from which we randomly sample (without replacement) throughout
training, typically processing over 80k image pairs.
We crop images to the bounding boxes provided with the dataset and, as with the CUB dataset, we resize 
images to $256\times256$. It is worth noting that Pascal VOC key-point is significantly more challenging than CUB as the native resolution of the image patches and the number of occluded key-points vary dramatically.  
% The maximum number of key-points in an image is 15.

\subsubsection{Sintel} This dataset is a synthetic video dataset with each frame having an attached ground truth optical flow map.
As in~\cite{Zanfir_CVPR18_DeepGM}, we split the original 23 training sequences first into 18 for training and the remaining of 5 for testing.
Each frame is split into 4$\times$4 sub images to be matched independently.
This dataset contains relatively small source to target displacements and less variance in appearance due to the nature of a pair of consecutive frames. However, the matching task in Sintel is dense and therefore poses a major challenge for the scalability of any tested method.

\subsection{CUB Results}

We first perform two sets of experiments on the CUB dataset to separately compare our results with both 
matching methods and graph matching methods.

In the first set, we adopt the standard PCK@$\alpha$ and EPE metric.
PCK is defined as the percentage of key-point predictions whose distances to the ground truth target key-points are closer than $\alpha\sqrt{w^2 + h^2}$, where $w$ and $h$ are the image width and height.
EPE~\cite{Butler_ECCV12_Sintel} is the end-to-end point error, which represents the mean $l^2$-norm error between predictions and ground truth.

In Fig.~\ref{fig:cubPCK}, we plot the PCK metric for $\alpha$ in the range 0.01 to 0.1.
The red curves represent our proposed approach. It can be seen that our method is significantly more accurate than the baselines when $\alpha<0.05$.
When $\alpha>0.05$, our method performs slightly worse than DeepGM because DeepGM directly regresses the target key-point location while our method regresses the assignment matrix. To better demonstrate the difference, we plot our method with the d-loss added (the red curve with dots), from which it can be seen that the d-loss regularises the network prediction, i.e. it improves the accuracy over the high $\alpha$ range at the cost of blurring the correct predictions, whilst remaining better than all of the other baseline approaches.  

In Table~\ref{tab:CUBresults}, we list the comparisons between our approach and several deep learning matching approach using both the EPE and PCK.
It can be seen that our method significantly outperforms the other deep 
learning methods. 

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.75\linewidth]{fig1.png}
    \caption{PCK@$\alpha$ results on the CUB dataset. The acronyms used in the figure are listed here. SIFT~\cite{Liu_PAMI11_SIFT}, DSF~\cite{Kin_CVPR13_DSF}, WarpNet~\cite{Kanazawa_CVPR16_WarpNet}, UCN~\cite{Choy_NIPS16_UCN}, DeepGM w VGG16 uses VGG16 as the feature extractor, and DeepGM w ResNet/FPN uses ResNet-50 and a feature pyramid network~\cite{Lin_CVPR17_PFN} as the feature extractor. }
    \label{fig:cubPCK}
\end{figure}

In the second set of experiments, we measure the precision and recall.
To validate the one-to-many results predicted by the network, we introduce the Many-to-One (MtO) score to quantify many-to-one errors.
MtO is defined as the sum of assignment occurrence divided by the total number of unique nodes, i.e. a score closer to 0 is better.

For this second set of experiments we compare our method with classical graph matching methods, including 
SM, IPFP, RRWM, NOGM, and MPM~\cite{Cho_CVPR14_MPM}. The input for GM is a set of 2D key-points, and the similarity matrix is calculated using $\exp(\frac{\|x_1 - x_2\|_2^2}{\sigma^2})$, with $\sigma=20\text{px}$; the graph is treated as fully connected. In contrast, the deep learning based approaches take as the input the deep feature vectors which contains image appearance clues.
To achieve a fair comparison with classical methods, we trained our method using the 2D key-point locations as the only features, i.e. the image feature extractor is removed and we use only 2 features rather than the full 258.
We average the precision and recall over the full test set.
The results of these experiments are shown in Table~\ref{tab:classicalresults}.
We can see that our method, even with pixel locations as features, outperforms all of the classic GM methods. We suggest that this can be attributed to the training. When combined with feature vectors that contain appearance clues and the orthogonal loss, our method achieves the best results and outperforms binarised DeepGM.
Binarised DeepGM takes the predicted assignment vector $\vect x$ as output and is binarised using the threshold 0.5. It serves to illustrate the matching performance of DeepGM without the displacement loss.

\begin{table}
\begin{minipage}{0.4\linewidth}
   \centering
   \resizebox{1\linewidth}{!}{
   \begin{tabular}{lrr}\toprule
   &\multicolumn{1}{l}{EPE}&\multicolumn{1}{l}{PCK @ $0.05$}\\
   \midrule
   UCN & 27.4 & 0.65 \\
   WarpNet & 21.1 & 0.83 \\
   NC-Net & 23.7 & 0.69 \\
   DeepGM w VGG-T & 17.0 & 0.86 \\
   DeepGM w Res-50 & 14.1 & 0.85 \\
   Ours  & 7.85   & 0.88 \\
   Ours w d-loss  & \textbf{7.39}   & \textbf{0.92} \\ \bottomrule
   \end{tabular}
   }
   \vspace{0.5em}
   \caption{Experimental results for the CUB dataset. The metrics are
   End-to-end Point Error (EPE, lower is better) and PCK (Higher is better).}
   \label{tab:CUBresults}
% \end{table}
\end{minipage}%
\hfill%
\begin{minipage}{0.55\linewidth}
% \begin{table}
   \centering
    \resizebox{\linewidth}{!}{
   \begin{tabular}{lrrr}\toprule
   &\multicolumn{1}{l}{Precision}&\multicolumn{1}{l}{Recall}&\multicolumn{1}{l}{MtO}\\
   \midrule
   SM   & 0.117 &  0.109 & \textbf{0.000}\\
   IPFP & 0.159 &  0.084 & \textbf{0.000}\\
   RRWM & 0.271  &  0.274 & 0.173\\
   NOGM & 0.263 &  0.323 & 0.132\\
   MPM & 0.212 &  0.212 & 0.321\\
   \vspace{1em}
   Ours w location only & 0.317 & 0.391 & 0.237\\
   Binarised DeepGM w ResNet & 0.482 & 0.490 & 0.384 \\
   Ours w/o orth loss & 0.645 & 0.427 & 0.361 \\
   \textbf{Ours} & \textbf{0.764} & \textbf{0.589} & 0.233\\\bottomrule
   \end{tabular}
    }
   \vspace{0.5em}
   \caption{Comparison of our results with selected classical GM approaches on the CUB dataset}
   \label{tab:classicalresults}
\end{minipage}
\end{table}

\subsection{PASCAL VOC Results}
For the matching test using the Pascal VOC key-point dataset, our network outperforms the 
state of the art by a large margin as shown in Table~\ref{tab:PASCALresults}.
We also evaluated against the PASCAL dataset using the learned weights from training with the CUB
dataset without any fine tuning, and the opposite way around (trained on PASCAL, tested against CUB).
Interestingly, we found that the network trained on PASCAL gave better results against CUB, than the
network trained on CUB when tested against PASCAL.
We suspect this may be due to the greater diversity of images in the PASCAL dataset, leading to a more
generally capable model, as well as the possibility of overfit in the model trained on CUB.
This suggests a future possible avenue of research, in investigating a class agnostic key-point matching approach.
Our selected qualitative results are shown in Fig.~\ref{fig:PASCALresults}.

\begin{table}
\begin{minipage}{0.45\linewidth}
   \centering
    \resizebox{\linewidth}{!}{
   \begin{tabular}{lrr}\toprule
   &\multicolumn{1}{l}{PCK @ $0.1$}\\
   \midrule
   SIFT flow     & 0.247 \\
   UCN           & 0.389 \\
   DeepGM w VGG  & 0.406 \\
   DeepGM w Res/FPN & 0.431 \\
   Ours (Trained on CUB)                & 0.356 \\
   \textbf{Ours}            & \textbf{0.519} \\\bottomrule
   \end{tabular}
    }%
   \vspace{0.5em}%
   \caption{Experimental results for the PASCAL VOC key-point dataset. 
   PCK (Higher is better) is averaged over all classes}%
   \label{tab:PASCALresults}%
% \end{table}%
\end{minipage}%
\hfill%
\begin{minipage}{0.45\linewidth}
% \begin{table}[h]%
   \centering
   \resizebox{1\linewidth}{!}{
   \begin{tabular}{lrr}\toprule
   &\multicolumn{1}{l}{PCK @10px}\\
   \midrule
    DeepGM [27] & 0.926\\
    DeepGM w ResNet/FPN & 0.933\\
    Ours & 0.917\\
    Ours w d-loss $\beta=0.5$ & 0.947\\\bottomrule
   \end{tabular}
   }
   \vspace{0.5em}
   \caption{Experimental results for Sintel using average PCK over all frames.}
   \label{tab:Sintel}
\end{minipage}
\end{table}

\begin{figure}[p]
    \centering
    \includegraphics[width=0.99\linewidth]{cub_challenging1.pdf}
    \caption{Predictions on the CUB dataset. From top to bottom: source image, target image, our prediction. Score in bottom right is MtO}
    \label{fig:orthocompareresults}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{pascalresults.pdf}
    \caption{Predictions on the PASCAL VOC dataset. From left to right (in threes): first image ground truth, second
    image ground truth, our prediction.}
    \label{fig:PASCALresults}
\end{figure}

\subsection{Sintel Results}
The test of scalability is mainly demonstrated using the Sintel dataset.
The issue with Sintel is universal to all GM approaches as the problem is NP hard. 
However, the reduced dimensionality of the affinity matrix means that our proposed method is faster than the main baseline when using the same backbone.
We demonstrate the capability of our approach by testing on MPI-Sintel which contains hundreds of nodes in each input image.
The results are detailed in Table~\ref{tab:Sintel}.


\subsection{Ablation Studies}
\label{sec:expabl}

The first set of the ablation tests concerns the performance of our orthogonal loss and the extra d-loss. In Fig.~\ref{fig:cubPCK}, we demonstrate that the PCK performance of our approach with the orthogonal loss (red) is consistently better than without (blue). 
The red curve with dots and the blue curve with dots represents the PCK performance with the d-loss. The visualisation of matching results with and without the orthogonal loss are shown in Fig.~\ref{fig:orthocompareresults}. It can be seen that MtO, shown in the bottom right corner of the figure, was effectively reduced by the orthogonal loss.

Regressing the target key-point location improves the performance of PCK accuracy for predictions that are relatively far from the target.
%, possibly because by comparing the training losses on the CUB dataset.
Using the orthogonal loss, we were able to achieve much higher precision and recall scores than
without. 


\begin{figure}[htb]
    \centering
    \includegraphics[width=0.85\linewidth]{orthogonal_loss.pdf}
    \caption{Predictions on CUB dataset. From left to right: source image, target
    image, our predictions with the Orthogonal loss, our predictions without the Orthogonal loss. The score in the bottom right is MtO}
    \label{fig:CUBresults}
\end{figure}


\subsection{Timing}
Regarding time efficiency, we compare between our method, DeepGM with the ResNet-50/FPN, and DeepGM with VGG. 
Importantly, we implement GM layers including the affinity layer, the power iteration layer and the bi-stochastic layer on top of the ResNet-50/FPN backbone.
The accuracy of the implementation on CUB is plotted as the black curve without dots in Fig.~\ref{fig:cubPCK}.
For one forward and backward pass, our approach is approximately 7$\times$ faster than DeepGM with ResNet-50/FPN.  
A single forward and backward pass using only our approach takes 0.043 seconds, an order
of magnitude faster than the original DeepGM with the VGG (0.447 seconds)
and about 7$\times$ faster that DeepGM with the ResNet/FPN feature extractor (0.307 seconds).
